EC-Net: an Edge-aware Point set Consolidation Network

Point clouds obtained from 3D scans are typically sparse, irregular, and noisy, and required to be consolidated. In this paper, we present the first deep learning based edge-aware technique to facilitate the consolidation of point clouds. We design our network to process points grouped in local patches, and train it to learn and help consolidate points, deliberately for edges. To achieve this, we formulate a regression component to simultaneously recover 3D point coordinates and point-to-edge distances from upsampled features, and an edge-aware joint loss function to directly minimize distances from output points to 3D meshes and to edges. Compared with previous neural network based works, our consolidation is edge-aware. During the synthesis, our network can attend to the detected sharp edges and enable more accurate 3D reconstructions. Also, we trained our network on virtual scanned point clouds, demonstrated the performance of our method on both synthetic and real point clouds, presented various surface reconstruction results, and showed how our method outperforms the state-of-the-arts.

==> related.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Related works
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

{\bf Related works.} \
Consolidating scanned data and imperfect point clouds has been an active research area since the early 90's~\cite{hoppe1992,turk-levoy-1994,amenta-1998}.
We briefly review some traditional geometric works and then discuss some recent related works that employ neural networks.
For a more comprehensive survey, please refer to~\cite{berger2017survey}.


\textit{Point cloud consolidation.} \
Early works in this area assumed smooth surface~\cite{alexa2003computing,lipman2007parameterization,huang2009consolidation}.
In~\cite{lipman2007parameterization}, the parameterization-free local projection operator (LOP) was devised to enhance the point set quality. 
However, these methods are oblivious to sharp edges and corners.
To consolidate a point set in an edge-aware manner, some methods detected/sensed the sharp edges and arranged points deliberatively along edges to preserve their sharpness~\cite{pauly2003shape,guennebaud2004real,fleishman2005robust,oztireli2009feature}.
Huang~\etal~\cite{huang2013edge} developed the edge-aware resampling (EAR) algorithm; it computes reliable normals away from edges and then progressively upsamples points towards the surface singularities.
Despite its promising results, EAR depends on the accuracy of the given/estimated normal.
Preiner~\etal~\cite{preiner2014continuous} developed CLOP, a continuous version of the LOP, for fast surface construction using the Gaussian mixture model to describe the point cloud density.
To sum up, these geometric approaches either assume strong priors or rely on extra geometric attributes for upsampling point sets.



\textit{Neural networks for mesh and point cloud processing.} \
Motivated by the promising results that deep learning methods have achieved for image and video problems, there has been increasing effort to leverage neural networks for geometry and 3D shape problems.
To do so, early works extracted low-level geometric features as inputs to CNNs~\cite{guo20153d,boulch2016deep}.
Other works converted the input triangular meshes or point clouds to regular voxel grids~\cite{Qi_2016_CVPR,dai2017complete,HRSC,wang2017cnn,Riegler2017OctNet,Liu_2017_ICCV} for CNN to process.
However, pre-extracting low-level features may bring bias, while a volume representation demands a high computational cost and is constrained by its resolution.

Recently, point clouds have drawn more attention, and there are some works to utilize neural networks to directly process point clouds. 
Qi~\etal~\cite{qi2017pointnet} firstly developed the PointNet, a network that takes a set of unordered points in 3D as inputs and learns features for object classification and segmentation.
Later, they proposed the PointNet++ to enhance the network with a hierarchical feature learning technique~\cite{qi2017pointnet++}.
Subsequently, many other networks have been proposed for high-level analysis problems with point clouds~\cite{hua2017pointwise,klokov2017escape,landrieu2017large,xu2017pointfusion,wang2017sgpn,qi2017frustum,li2018pointcnn,wang2018dynamic,su2018splatnet}.
However, they all focus on analyzing global or mid-level attributes of point clouds.
In some other aspects, Guerrero~\etal~\cite{guerrero2017pcpnet} proposed a network to estimate the local shape properties in point clouds, including normal and curvature.
3D reconstruction from 2D images has also been widely studied~\cite{Groueix2018AtlasNet,Fan_2017_CVPR,lin2017learning}.
Our work is most related to PU-Net~\cite{yu-2018-pu-net}, which presented a network to upsample a point set. However, our method is edge-aware, and we extract local patches and train the network to learn edges in patches with a novel edge-aware joint loss function.

